Integration of Preferences in Decomposition Multi-Objective Optimization

Most existing studies on evolutionary multi-objective optimization focus on approximating the whole Pareto-optimal front. Nevertheless, rather than the whole front, which demands for too many points (especially in a high-dimensional space), the decision maker might only interest in a partial region, called the region of interest. In this case, solutions outside this region can be noisy to the decision making procedure. Even worse, there is no guarantee that we can find the preferred solutions when tackling problems with complicated properties or a large number of objectives. In this paper, we develop a systematic way to incorporate the decision maker's preference information into the decomposition-based evolutionary multi-objective optimization methods. Generally speaking, our basic idea is a non-uniform mapping scheme by which the originally uniformly distributed reference points on a canonical simplex can be mapped to the new positions close to the aspiration level vector specified by the decision maker. By these means, we are able to steer the search process towards the region of interest either directly or in an interactive manner and also handle a large number of objectives. In the meanwhile, the boundary solutions can be approximated given the decision maker's requirements. Furthermore, the extent of the region of the interest is intuitively understandable and controllable in a closed form. Extensive experiments, both proof-of-principle and on a variety of problems with 3 to 10 objectives, fully demonstrate the effectiveness of our proposed method for approximating the preferred solutions in the region of interest.

==> proofprinciple.tex <==
% !tex root = main.tex

\section{Proof-of-Principle Experiments}
\label{sec:proofofprinciple}

Generally speaking, the proof-of-principle experiments are divided into four parts. First of all, we validate the effectiveness of the NUMS with respect to various aspiration level vector settings. Afterwards, we empirically investigate some interesting extensions of the NUMS for handling various scenarios, i.e., problems with a large number of objectives, multiple ROIs and an interactive preference incorporation, step by step.%At last, we apply NUMS to several other state-of-the-art decomposition-based EMO algorithms and compare their abilities to search for the ROIs.

For proof-of-principle purpose, our recently developed MOEA/D variant based on the stable matching model~\cite{GSmethod}, named MOEA/D-STM~\cite{MOEAD-STM}, is employed as the baseline algorithm. Different from the canonical MOEA/D, where the selection of the next parents is merely determined by the aggregation function value of a solution, MOEA/D-STM treats subproblems and solutions as two sets of agents and considers their mutual-preferences simultaneously. In particular, the preference of a subproblem over a solution measures the convergence issue, while the preference of a solution over a subproblem measures the diversity issue. Since the stable matching achieves an equilibrium of the mutual-preferences between subproblems and solutions, MOEA/D-STM strikes a balance between convergence and diversity of the search process. Here we use simulated binary crossover (SBX)~\cite{SBX} and polynomial mutation~\cite{PolyMutation} as the reproduction operators. For the SBX, its crossover probability is set as $p_c=1.0$ and its distribution index is set as $\eta_c=10$; for the polynomial mutation, its mutation probability is set as $p_m=\frac{1}{n}$ and its distribution index is set as $\eta_m=20$.%ZDT~\cite{ZDT} and DTLZ~\cite{DTLZ} test suites are chosen to form the benchmark.


\subsection{Proof-of-Principle Results}
\label{sec:proof}

Let us start from the two-objective test problem ZDT1 which has a convex PF~\cite{ZDT}. The population size is set to 100 and the number of function evaluations is set to 30,000. \pref{fig:proof_ZDT1} shows a comparative results of solutions obtained by MOEA/D-STM with different $\tau$ settings. From this figure, we clearly see that the NUMS adapts the originally uniformly distributed reference points to a biased distribution with a required extent. Accordingly, MOEA/D-STM provides a well approximation of the partial PF with respect to these biased reference points. Note that, in order to approximate the whole PF without preferences on any particular region, we need to set $\tau=1-\frac{2}{99}$ rather than 1.0 according to \pref{theorem:eta}. Next, we assess the performance of MOEA/D-STM with the NUMS on the three-objective test problems DTLZ1 and DTLZ2 respectively. In particular, 30,000 function evaluations are used for DTLZ2 and 100,000 function evaluations are used for DTLZ1 due to its multimodality. As shown in~\pref{fig:proof_DTLZ1} and \pref{fig:proof_DTLZ2}, with either an infeasible ($\mathbf{z}^r=(0.3,0.3,0.2)^T$ for DTLZ1) or feasible ($\mathbf{z}^r=(0.3,0.5,0.6)^T$ for DTLZ2) aspiration level vector, MOEA/D-STM has no difficulty in finding solutions crowded around the ROI. In addition, MOEA/D-STM also well approximates the boundaries for both DTLZ1 and DTLZ2. At last, let us consider a five-objective DTLZ2 problem with $\mathbf{z}^r=(0.3,0.1,0.4,0.2,0.3)^T$ as the aspiration level vector. Now, we set $H=7$ in the Das and Dennis's method which generates 330 uniformly distributed reference points, and $\tau$ is set to 0.1 in NUMS. \pref{fig:proof_5D}(c) gives the theoretical optimal points, with respect to the adapted reference points given in~\pref{fig:proof_5D}(b), on the PF of DTLZ2, according to the method developed in~\cite{MOEADD}. Comparing \pref{fig:proof_5D}(a) with \pref{fig:proof_5D}(c), we can see that MOEA/D-STM, after performing 330,000 function evaluations, has a well approximation to both the ROI and the boundary points.

\begin{figure*}[htbp]
\centering

\pgfplotsset{every axis/.append style={
%% font = \Large,
grid = major,
xlabel = {$f_1$},
ylabel = {$f_2$},
xmin = 0, xmax = 1.001,
ymin = 0, ymax = 1.005,
%% mark options = {mark size = 2.0},
%% ymode  = log,
thick,
line width = 1pt,
tick style = {line width = 0.8pt}}}

  \subfloat[$\tau=0.1$]{
  \resizebox{0.25\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}[
      legend columns = -1,
      legend style   = {font=\scriptsize},
      legend entries = {PF, r-MOEA/D-STM, reference points, $\mathbf{z}^r$= {(0.3, 0.4)}},
      legend to name = named
      ]
		\addplot[very thick, gray, mark = none] table {Data/PF/ZDT1.dat};
    \addplot[only marks, thick, black, mark = *] table {Data/ZDT4/t1.dat};
    \addplot[only marks, thick, gray, mark = o] table {Data/refp/pW2D_ZDT4_1.dat};
    \addplot[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.3, 0.4)};
	\end{axis}
      \end{tikzpicture}
    }}
  \subfloat[$\tau=0.3$]{
  \resizebox{0.25\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}
    \addplot[very thick, gray, mark = none] table {Data/PF/ZDT1.dat};
    \addplot[only marks, thick, black, mark = *] table {Data/ZDT4/t3.dat};
    \addplot[only marks, thick, gray, mark = o] table {Data/refp/pW2D_ZDT4_3.dat};
    \addplot[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.3, 0.4)};
	\end{axis}
      \end{tikzpicture}
    }}
  \subfloat[$\tau=0.7$]{
  \resizebox{0.25\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}
    \addplot[very thick, gray, mark = none] table {Data/PF/ZDT1.dat};
    \addplot[only marks, thick, black, mark = *] table {Data/ZDT4/t7.dat};
    \addplot[only marks, thick, gray, mark = o] table {Data/refp/pW2D_ZDT4_7.dat};
    \addplot[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.3, 0.4)};
	\end{axis}
      \end{tikzpicture}
    }}
  \subfloat[$\tau=0.9798$]{
  \resizebox{0.25\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}
    \addplot[very thick, gray, mark = none] table {Data/PF/ZDT1.dat};
    \addplot[only marks, thick, black, mark = *] table {Data/ZDT4/t10.dat};
    \addplot[only marks, thick, gray, mark = o] table {Data/refp/pW2D_ZDT4_10.dat};
    \addplot[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.3, 0.4)};
	\end{axis}
      \end{tikzpicture}
    }}

\ref{named}
\caption{Comparisons of solutions obtained by MOEA/D-STM with different $\tau$ settings for NUMS on ZDT1 problems}
\label{fig:proof_ZDT1}
\end{figure*}

\begin{figure}[htbp]
\centering

\pgfplotsset{every axis/.append style={
%% font = \Large,
grid = major,
view   = {135}{30},
xlabel = {$f_1$},
ylabel = {$f_2$},
zlabel = {$f_3$},
xmin = 0, xmax = 1.001,
ymin = 0, ymax = 1.005,
zmin = 0, zmax = 1.005,
%% mark options = {mark size = 2.0},
%% ymode  = log,
thick,
line width = 1pt,
tick style = {line width = 0.8pt}}}

  \subfloat[$\tau=0.3$]{
  \resizebox{0.25\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}[
      legend columns = -1,
      legend style   = {font=\scriptsize},
      legend entries = {r-MOEA/D-STM, reference points, $\mathbf{z}^r$= {(0.3, 0.3, 0.2)}},
      legend to name = named1
      ]
    \addplot3[only marks, thick, black, mark = *] table {Data/DTLZ1/t3.dat};
    \addplot3[only marks, thick, gray, mark = o] table {Data/refp/pW3D_DTLZ1_3.dat};
    \addplot3[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.3, 0.3, 0.2)};
	\end{axis}
      \end{tikzpicture}
    }}
  \subfloat[$\tau=0.3$]{
  \resizebox{0.25\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}[
    view = {45}{30}
    ]
    \addplot3[only marks, thick, black, mark = *] table {Data/DTLZ1/t3.dat};
    \addplot3[only marks, thick, gray, mark = o] table {Data/refp/pW3D_DTLZ1_3.dat};
    \addplot3[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.3, 0.3, 0.2)};
	\end{axis}
      \end{tikzpicture}
    }}

\ref{named1}
\caption{Solutions obtained by MOEA/D-STM on DTLZ1 problem where $\mathbf{z}^r=(0.3, 0.3, 0.2)$.}
\label{fig:proof_DTLZ1}
\end{figure}

\begin{figure}[htbp]
\centering

\pgfplotsset{every axis/.append style={
%% font = \Large,
grid = major,
view   = {135}{30},
xlabel = {$f_1$},
ylabel = {$f_2$},
zlabel = {$f_3$},
xmin = 0, xmax = 1.001,
ymin = 0, ymax = 1.005,
zmin = 0, zmax = 1.005,
%% mark options = {mark size = 2.0},
%% ymode  = log,
thick,
line width = 1pt,
tick style = {line width = 0.8pt}}}

  \subfloat[$\tau=0.3$]{
  \resizebox{0.25\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}[
      legend columns = -1,
      legend style   = {font=\scriptsize},
      legend entries = {r-MOEA/D-STM, reference points, $\mathbf{z}^r$= {(0.3, 0.5, 0.6)}},
      legend to name = named2
      ]
		% \addplot[very thick, gray, mark = none] table {Data/PF/ZDT1.dat}; 
    \addplot3[only marks, thick, black, mark = *] table {Data/DTLZ2/t3.dat};
    \addplot3[only marks, thick, gray, mark = o] table {Data/refp/pW3D_DTLZ2_3.dat};
    \addplot3[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.2, 0.5, 0.6)};
	\end{axis}
      \end{tikzpicture}
    }}
  \subfloat[$\tau=0.3$]{
  \resizebox{0.23\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}[
    view = {75}{30}
    ]
    % \addplot[very thick, gray, mark = none] table {Data/PF/ZDT1.dat};
    \addplot3[only marks, thick, black, mark = *] table {Data/DTLZ2/t3.dat};
    \addplot3[only marks, thick, gray, mark = o] table {Data/refp/pW3D_DTLZ2_3.dat};
    \addplot3[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.2, 0.5, 0.6)};
	\end{axis}
      \end{tikzpicture}
    }}

\ref{named2}
\caption{Solutions obtained by MOEA/D-STM on DTLZ2 problem where $\mathbf{z}^r=(0.2, 0.5, 0.6)^T$.}
\label{fig:proof_DTLZ2}
\end{figure}

\begin{figure*}
\centering
\subfloat[MOEA/D-STM.]{\includegraphics[width=.33\linewidth]{Figures/proof5D.eps}}
\subfloat[Reference points.]{\includegraphics[width=.33\linewidth]{Figures/proofweight5D.eps}}
\subfloat[Theoretical optima.]{\includegraphics[width=.33\linewidth]{Figures/PF_5D.eps}}
\caption{Solutions obtained by MOEA/D-STM on 5-objective DTLZ2 problem where $\mathbf{z}^r=(0.3, 0.1, 0.4, 0.2, 0.3)^T$.}
\label{fig:proof_5D}
\end{figure*}

\subsection{Problems with a Large Number of Objectives}
\label{sec:manyobjs}

As discussed in~\cite{MOEADD} and~\cite{NSGA-III}, in order to have intermediate reference points within the simplex, we should set $H\geq m$ in the Das and Dennis's method. Otherwise, all reference points should lie on the boundary of the simplex. However, in a large-dimensional space, we can have a huge amount of reference points even when $H=m$. For example, when $m=10$, the Das and Dennis's method can generate $\binom{10+10-1}{10-1}=92378$ uniformly distributed reference points if $H=10$. Obviously, current EMO algorithms cannot hold such huge number of solutions in a population. Even worse, when $H=m$, there is only one intermediate reference point which lies in the center of the simplex. This means that the original NUMS might not be directly applicable when facing a large number of objectives. Inspired by the multi-layer weight vector generation method developed in~\cite{MOEADD} and~\cite{NSGA-III}, we make a slight modification to adapt the NUMS to the many-objective scenario. First of all, we use the Das and Dennis's method, where $H<m$, $l$ times ($l>1$) to generate $l$ layers of reference points. Afterwards, we use the method developed in~\pref{sec:boundary} to shift these reference points, which lie on the boundary, onto the ROI layer by layer. \pref{fig:proof_10D}(b) shows an example of 661 reference points generated by the multi-layer NUMS where the aspiration level vector is set as $\mathbf{z}^r=(0.3, 0.3, 0.3, 0.1, 0.3, 0.55, 0.35, 0.35, 0.25, 0.45)^T$. In particular, we first use the Das and Dennis's method to generate $l=3$ layers of reference points. Since we set $H=3$, each layer contains 220 reference points. Then two layers of them are shifted onto the ROI, where the shrinkage factor $\tau$ is set to 0.4 and 0.2 respectively. \pref{fig:proof_10D}(a) shows the final solutions obtained by MOEA/D-STM after 661,000 generations. Comparing to the theoretical optima shown in~\pref{fig:proof_10D}(c), we can see that MOEA/D-STM has a satisfied approximation to the ROI in a 10-objective scenario.

\begin{figure*}
\centering
\subfloat[r-MOEA/D-STM.]{\includegraphics[width=.33\linewidth]{Figures/proof10D.eps}}
\subfloat[Reference points.]{\includegraphics[width=.33\linewidth]{Figures/proofweight10D.eps}}
\subfloat[Theoretical optima.]{\includegraphics[width=.33\linewidth]{Figures/PF_10D.eps}}
\caption{Solutions obtained by MOEA/D-STM on 10-objective DTLZ2 problem where $\mathbf{z}^r=(0.3, 0.3, 0.3, 0.1, 0.3, 0.55, 0.35, 0.35, 0.25, 0.45)^T$.}
\label{fig:proof_10D}
\end{figure*}

\subsection{Investigations on multiple ROIs}
\label{sec:multipleROIs}

In practice, the DM might not be sure about his/her exact preferences and he/she would like to simultaneously explore several ROIs. In this case, the DM would like to supply more than one, say $T>1$, aspiration level vectors simultaneously. To accommodate multiple ROIs, we only need to apply the NUMS $T$ times with respect to each aspiration level vector. Note that each time the NUMS can preserve the boundary reference points, but we only need to keep these boundary reference points once. In other words, the duplicated boundary reference points are exempted from the final reference point set. \pref{fig:proof_DTLZ2double} shows an example of two aspiration level vectors. In particular, the gray points are the adapted reference points for each ROI; while the black points are the final solutions obtained by MOEA/D-STM with respect to the corresponding reference points. From the experimental results, we can clearly see that MOEA/D-STM with the NUMS is also able to approximate multiple ROIs simultaneously.

\begin{figure}[htbp]
\centering

\pgfplotsset{every axis/.append style={
%% font = \Large,
grid = major,
view   = {135}{30},
xlabel = {$f_1$},
ylabel = {$f_2$},
zlabel = {$f_3$},
xmin = 0, xmax = 1.001,
ymin = 0, ymax = 1.005,
zmin = 0, zmax = 1.005,
%% mark options = {mark size = 2.0},
%% ymode  = log,
thick,
line width = 1pt,
tick style = {line width = 0.8pt}}}

  \subfloat[$\tau=0.3$]{
  \resizebox{0.25\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}[
      legend columns = -1,
      legend style   = {font=\scriptsize},
      legend entries = {MOEA/D-STM, reference points, $\mathbf{z}^{r1}$= {(0.3, 0.5, 0.7)}, $\mathbf{z}^{r2}$= {(0.9, 0.3, 0.3)}},
      legend to name = named3
      ]
    \addplot3[only marks, thick, black, mark = *] table {Data/DTLZ2/t2_double.dat};
    \addplot3[only marks, thick, gray, mark = o] table {Data/refp/pW3D_DTLZ2_double.dat};
    \addplot3[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.2, 0.5, 0.7)};
    \addplot3[only marks, thick, blue, mark size = 3.0, mark = Mercedes star] coordinates {(0.9, 0.3, 0.3)};
	\end{axis}
      \end{tikzpicture}
    }}
  \subfloat[$\tau=0.3$]{
  \resizebox{0.23\textwidth}{!}{
      \begin{tikzpicture}
	\begin{axis}[
    view = {75}{30}
    ]
    \addplot3[only marks, thick, black, mark = *] table {Data/DTLZ2/t2_double.dat};
    \addplot3[only marks, thick, gray, mark = o] table {Data/refp/pW3D_DTLZ2_double.dat};
    \addplot3[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.2, 0.5, 0.7)};
    \addplot3[only marks, thick, blue, mark size = 3.0, mark = Mercedes star] coordinates {(0.9, 0.3, 0.3)};
	\end{axis}
      \end{tikzpicture}
    }}

\ref{named3}
\caption{Solutions obtained by MOEA/D-STM with two different reference points on DTLZ2 problem.}
\label{fig:proof_DTLZ2double}
\end{figure}

\subsection{Interactive Scenario}
\label{sec:interactive}

In the real-world optimization, the DM is usually not fully confident about his/her elucidated preference information due to the lack of the knowledge of the PF beforehand. Therefore, an interactive decision making procedure, by which the DM can progressively adapt his/her preference information during the optimization process, is attractive in the preference-based EMO. Since the NUMS can easily adapt the distribution of reference points to be biased towards the ROI, it facilitates the interactive decision making procedure. Moreover, also due to the lack of the knowledge of the PF, the DM can easily specify an aspiration level vector which is far away from the boundary of the PF. Since the NUMS is able to preserve the reference points lying on the boundary, it finally helps the DM better understand the PF (e.g., its geometric characteristics and ideal/nadir point) and revise his/her preference information. In~\pref{fig:interactive}, we describe an interactive run, which includes three cycles, of MOEA/D-STM on DTLZ2. We call a run of the MOEA/D-STM for a certain number of function evaluations specified by the DM as a cycle. At the beginning, as shown in~\pref{fig:interactive}(a), the DM specifies an aspiration level vector $\mathbf{z}^r_1=(1.4,1.9,1.5)^T$ far away from the PF. After 20,000 function evaluations, MOEA/D-STM finds the solutions not only crowd in the ROI, but also distribute along the boundary. Thereafter, the DM realizes that $\mathbf{z}^r_1$ is a bad choice, and then he/she resets the aspiration level vector as $\mathbf{z}^r_2=(0.7,0.6,0.3)^T$. In addition, since the DM already knows the boundary of the PF, he/she might not be interested in it any longer. Thus, he/she sets the NUMS to adapt all reference points to the ROI. By using the final population of the first interaction as the initial population, MOEA/D-STM finally find the solutions in the ROI after 20,000 function evaluations. However, we assume that the DM still does not satisfy them and further revise the aspiration level vector as $\mathbf{z}^r_3=(0.3, 0.4, 0.8)^T$. After another 20,000 function evaluations, as shown in~\pref{fig:interactive}(c), MOEA/D-STM finds the solutions in the vicinity of the ROI.


\begin{figure*}[htbp]
\centering

\pgfplotsset{every axis/.append style={
%% font = \Large,
grid = major,
view   = {75}{30},
xlabel = {$f_1$},
ylabel = {$f_2$},
zlabel = {$f_3$},
xmin = 0, xmax = 1.001,
ymin = 0, ymax = 1.005,
zmin = 0, zmax = 1.005,
%% mark options = {mark size = 2.0},
%% ymode  = log,
thick,
line width = 1pt,
tick style = {line width = 0.8pt}}}

\subfloat[1st interaction]{
  \resizebox{0.33\textwidth}{!}{
\begin{tikzpicture}
\begin{axis}[
  legend columns = -1,
  legend style   = {font=\scriptsize},
  legend entries = {r-MOEA/D-STM, reference points},
  legend to name = named4,
  xmax = 2.000,
  ymax = 2.000,
  zmax = 2.000
  ]
  \addplot3[only marks, thick, black, mark = *] table {Data/IN/FUN0.dat};
  \addplot3[only marks, thick, gray, mark = o] table {Data/refp/pW3D_DTLZ2_IN_1.dat};
  \addplot3[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(1.4, 1.9, 1.5)};
\end{axis}
\end{tikzpicture}
}}
\subfloat[2nd interaction]{
  \resizebox{0.33\textwidth}{!}{
\begin{tikzpicture}
\begin{axis}
  \addplot3[only marks, thick, black, mark = *] table {Data/IN/FUN1.dat};
  \addplot3[only marks, thick, gray, mark = o] table {Data/refp/pW3D_DTLZ2_IN_2.dat};
  \addplot3[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.7, 0.6, 0.3)};
\end{axis}
\end{tikzpicture}
}}
\subfloat[3rd interaction]{
  \resizebox{0.33\textwidth}{!}{
\begin{tikzpicture}
\begin{axis}
  \addplot3[only marks, thick, black, mark = *] table {Data/IN/FUN2.dat};
  \addplot3[only marks, thick, gray, mark = o] table {Data/refp/pW3D_DTLZ2_IN_3.dat};
  \addplot3[only marks, thick, red, mark size = 3.0, mark = star] coordinates {(0.3, 0.4, 0.8)};
\end{axis}
\end{tikzpicture}
}}

\ref{named4}
\caption{Interactive scenario on DTLZ2 problem.}
\label{fig:interactive}
\end{figure*}

